Interactive Learning with Pricing for Optimal and Stable Allocations in Markets

Large-scale online recommendation systems must facilitate the allocation of a limited number of items among competing users while learning their preferences from user feedback. As a principled way of incorporating market constraints and user incentives in the design, we consider our objectives to be two-fold: maximal social welfare with minimal instability. To maximize social welfare, our proposed framework enhances the quality of recommendations by exploring allocations that optimistically maximize the rewards. To minimize instability, a measure of users' incentives to deviate from recommended allocations, the algorithm prices the items based on a scheme derived from the Walrasian equilibria. Though it is known that these equilibria yield stable prices for markets with known user preferences, our approach accounts for the inherent uncertainty in the preferences and further ensures that the users accept their recommendations under offered prices. To the best of our knowledge, our approach is the first to integrate techniques from combinatorial bandits, optimal resource allocation, and collaborative filtering to obtain an algorithm that achieves sub-linear social welfare regret as well as sub-linear instability. Empirical studies on synthetic and real-world data also demonstrate the efficacy of our strategy compared to approaches that do not fully incorporate all these aspects.

==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We pose the problem of making recommendations that will achieve optimal allocations in markets with constraints. Then, we formulate this problem as a structured combinatorial bandit and propose a no-regret algorithm.}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{learning_opt_alloc}, we describe that we are studying the posed problem of interactive recommendations for optimum allocations under the assumptions that facilitate our theoretical analysis. In Section \ref{sect_lrcb}, we indicate that one possible approach to improve upon our theoretical analysis might be by assuming a problem setting where at most some specific number of the arms can be played in each round.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Assumptions \ref{rew_assumptio} and \ref{low_assum} in Section \ref{sect_methodology}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix \ref{appendix_num}, \ref{SCMAB}, \ref{pf_conf_sets}, \ref{pf_regrets} and \ref{pf_allocation}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and data for the simulations are provided in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The hyperparameters of experimental settings are given in  Appendix \ref{sect_additional_exp} as well as the captions of Figures \ref{fig_regrets} and \ref{fig_cap}. Further implementation details can be found in the code.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Figure \ref{fig_regrets} and other figures in Appendix \ref{sect_additional_exp}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{sect_additional_exp}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{The datasets are cited appropriately.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The code and data for the simulations are provided in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tex/discussion.tex <==
%!TEX root = ../main.tex

\section{Discussion}
\label{sec:discussion}

Describe how recommendations have become an integral part of our socioeconomic life.
Describe how the current implementations miss the key factor of limited service capacities.
Use examples such as restaurant suggestions, hospital suggestions, supply chain recommendations and business decisions.
Our goal is to design a recommendation system that is aware of market conditions, service capacities, etc.


El Farol Bar, Kolkata Paisa Restaurant problem, etc (mainly statistical methods in this literature).
Learning related works: Include the paper found by Efe related to such works, paper by Jordan, etc. 
Show what is missing in each one of them. 
For example, pricing, or capacity constraints, or utilities, etc.
Kelly handles many of these aspects but lacks learning efficiciency.
For example, there is a huge communication overhead involved in signalling between the network and the users.


% Setting in short - elaborate on this later
We consider the setting of online food delivery as an example setting to demonstrate our approach.
Consider a platform that allocates diners to restaurants.
(Doordash and UberEats are prominent examples of such platforms today.)
Diners come to the platform seeking to place orders.
There are several restaurants registered with the platform ready to serve. 
Besides there are people who deliver the food from the restaurants to the diners.
Other possible participants include the stakeholders, regulatory agencies, worker unions, etc.
This classification is useful to characterize the relevant attributes that are related to the different components in the network and how they connect with each other. 

Here is an example of the relevant attributes and their inter-connectedness.
The diners have preferences over the different restaurants.
Along with the food choice, the diners also care about the delay in their service, i.e.
the time it takes for them to recieve their order.
Preference over restaurants and delays is an important attribute of the diners.
These preferences are their private knowledge which might be hard to learn with limited communication.
Besides the diners might also be unwilling to report these truthfully.
We allow different diners to have different preferences, but they all belong to the same class of having preferences over restaurants and delays.
On the other hand, the restaurants have different serving capacities.
The number of diners that are being served 
by any given restaurant affects the delay of the diners served by that restaurant 
and in turn the experience of these diners.


There are several more aspects to this problem, for example, the availability of delivery people affects the delays.
The delivery people will have different preferences over where they wish to travel in order to deliver.
For example, at the end of the day a delivery person would prefer to deliver at a place closer to her home.
The restaurants can also have preferences over their idle times, for example, different restaurants would care differently about the lack of orders.
For example, restaurants that have online food delivery as their main source of revenue will care more whereas restaurants that rely more on on-foot traffic to their restaurants will care less.
Besides, it is a dynamic setting since the availability of delivery people, the preferences of the agents in the network, and the serving capacities of the restaurants are all changing with time.
We will take a market-based approach to solve this problem.


In this paper, however, we will restrict our attention to serving the diners to the best extent possible given the constraints coming from the limited serving capacities of the restaurants and the availability of delivery persons.
We will only care about the preferences of the diners and treat the other components of the network as capacity constraints.
We will relegate the more general problem incorporating the preferences of the other components in the network for future papers.

\subsection{Notes from Intro}




Our approach is based on integrating methods from network economics (Kelly decentralized network framework) with collaborative filtering (for example, matrix factorization or latent variable models) and bandits learning (for example, UCB or Thompson sampling). 
% The resource allocation in these markets is enhanced by the use of fast communication channels provided by the internet and the ability to collect extensive data and use computational tools to perform learning tasks.
% Our integrated framework will provide a systematic way to combine these instruments for optimal resource allocation and real-time price discovery with limited user interaction.
% Objective in short - elaborate on this later
Our framework can be thought of as an extension of the market based methods in 
network resource allocation settings with the additional feature of practical limitations in collecting the required information.
This requires striking a balance between opportunistically learning the unknown preferences and allocating the limited items.


Intuition:
In market settings prices naturally adjust to the demand and the preferences of the agents so that 
we allocate items to the agents that prefer them the most.
Kelly proposed a framework in the context of bandwidth allocation over the Internet.
The system consists of users with preferences and limited resources that can be used to serve the users.
The users preferences are modeled as utility functions over their outcomes,
and the outcomes are a function of the resource allocation in the system.
The problem is formulated as a social welfare maximization one (or equivalently customer satisfaction maximization) subject to the capacity constraints in the system.
Often, the system operator (platform) does not know the user preferences, only the users know their own preferences (or at least have an idea about it).
On the other hand the users do not know about the system capacity constraints and the system operator is best placed to collect this information.
% The decentralized approach allows us to solve this problem through appropriate market pricing scheme that also adapts to the changing environment provided the change is slow enough (do experiments for this point).



In theory, the above framework should solve our problem.
However, in the framework proposed by Kelly, 
we would require the agents to respond constantly with their updated bids for different items.
Given how large the number of available items can be, 
it is impractical to get such responses from the agents.
Assuming that the agents preferences are related to each other with a hidden low dimensional structure,
it is natural to use methods from collaborative filtering  to resolve this problem.


\subsection{EXtending to dynamic settings}

Let $[n] := \{1, 2, \dots, n\}$ be the set of diners, with a typical diner denoted by $i$.
Let $[m] := \{1, 2, \dots, m\}$ be the set of restaurants, with a typical restaurant denoted by $r$.
For each diner, restaurant pair let $u_{i,r}:\bbR^+ \to \bbR^+$ be the utility function, where $u_{i,r}(\tau)$ denotes the utility diner $i$ gets from ordering from restaurant $r$ with a service delay of time $\tau > 0$.


As in the serverless pricing paper, we will dicretize the delay times into several tiers or levels.
Let $[l] := \{1, 2, \dots, l\}$ be the set of delay tiers with a typical tier denoted by $t$.
For example, let tier $1$ correspond to a delay of at most $10$ mins, tier $2$ correspond to a delay or more than $10$ mins and less than $30$ mins, tier 3 correspond to a delay of more than $30$ mins and less than $60$ mins, and so on.
Note that the intervals in the different tiers can be of different lengths.
Our framework is general enough to model any of these.
The more the number of intervals, the higher precision we have over the utility functions, but it makes the computational problem harder leading to greater estimation and approximation errors.
Thus, the design of tiers is an important practical problem and will depend on the particular setting and tradeoff concerns.
We will assume that we have 6 tiers, each with a length of $10$ mins.
Thus, the maximum delay that we allow is $1$ hr beyond which we assume that the utility is $0$.

(Include a diagram of utility function and values corresponding to tiers.)


Let $U$ be an $n \times m \times l$ tensor, where $U(i,r,t)$ is the utility of diner $i$ if she receives her order from restaurant $r$ within the delay tier $t$.
This models the preferences of the diners.
Let us now model the system constraints.
We will first have a stylized model for the system, but then relax it later.
Let $\mu_r$ denote the average service rate of restaurant $r$, i.e. if $\mu_r = 1$ serving/min then restaurant $r$ can cook 1 serving every min on average.
Given the current availability of delivery persons, let $\delta_{i,r}$ denote the time it takes to deliver the order from restaurnat $r$ to diner $i$.
Let us assume that this is also fixed for the moment, for example, say we use the average delay in delivery time.
(The general RL framework will be stronger and be able to adapt to changing delivery times and restaurant serving rates. In that case we won't assume that we know these values a priori, but the RL framework will learn and predict these values in an online fashion.)



I will now describe the dynamic aspect in this problem.
We envision the scheduler to operate periodically, say every $1$ min.
Let us descritize the time into $1$ min intervals and starting at time $s = 0$.
At any instant, it maintains a queue of orders that are yet to be scheduled.
To elaborate, diners come to our platform and enter their order size. 
The diners who are currently looking to order from our platform will be called active diners.
Let $A(s) \subset [n]$ denote the set of active diners at step $s$.
Each diner $i$ once it comes to the platform, inputs its order size $J_i$, the amount of food she wishes to order.
Thus for each active diner, i.e. $i \in A$, we know the order size $J_i$.


On the operation of the scheduler in step $s$ it comes up with a matching restaurant for each customer, a corresponding delay in service, and the corresponding cost for the order.
(I will soon describe how the scheduler comes up with these allocations and pricing, but it is similar to the static scheduler in the serverless pricing paper.)
Each active diner observes this suggestion and either accepts it or rejects it.
If the diner accepts the suggestion, she is scheduled for that order and removed from the queue and is not an active diner anymore.
(I will use the queue and the set of active diners interchangeably, since they are identical in this framework.)
If the diner does not accept the suggestion, she is kept in the queue and will get a new suggestion in the next operation of the scheduler.
(Possible considerations for practical reasons: we don't want to make the diners wait for $1$ min to come up with a new suggestion. We can consider providing multiple suggestions in each iteration to each diner, or a scheduler that operates at a faster time-scale.)


Let the amount of food allocated to user $i$ from restaurant $r$ in tier $t$ by the scheduler be denoted by $x(i,r,t)$.
The static problem that the scheduler solves at every operation can be stated as follows:

\begin{align}
\text{\bf\underline{SYS}} \nn \\
\maxi_{x(i,r,t)\geq 0} ~~~~~& \sum_{i=1}^n U(i,R_i,T_i)\nn \\
\text{subject to} ~~~~~& \sum_{i = 1}^N x(i,r,t) \leq M(r,t), \forall~ r \in [m], t \in [l], \text{ and }\label{eq: sys_capacity}\\
& R_i, T_i \in \left\{(r,t) \in [m]\times[l]: \sum_{s = 1}^t x(i,r,s) \geq J_i\right\} ~\forall~ i \in [n].
 % & T_i = \min \{t \in [T] : \sum_{s = 1}^t x_{i,s} \geq J_i \}, ~\forall~ i \in [N]. 
 \label{eq: sys_T_def}
\end{align}


Let
\[
	F(i,r,t) = \frac{U(i,r,t)}{J_i}.
\]
We relax the above system problem as follows:

\begin{align}
\text{\bf \underline{SYS-LP}}\nn\\
\maxi_{x(i,r,t)\geq 0} ~~~~~&\sum_{i=1}^N \sum_{t=1}^T x(i,r,t)F(i,r,t)\nn \\
\text{subject to} ~~~~~&\sum_{t=1}^T \sum_{r = 1}^m x(i,r,t) \leq J_i, ~\forall ~i \in [N], \label{tot_job_cons}\\
&\sum_{i = 1}^N x(i,r,t) \leq M(r,t), ~\forall~ r \in [m], t \in [l]. \label{tot_resource_cons}
% & x_{it} \geq 0, ~\forall~ i \in [N], t \in [T]\nn.
\end{align}


This is an LP problem and can be solved efficiently.
(By performing sparcity analysis we should show that for most of the users their orders come from a single restaurant in a single tier. 
Use this to provide a bound for the relaxation.)
Further, we can use Kelly decomposition on this relaxed system problem to obtain a decentralized version for solving this problem.
It also gives rise to price discovery $p(i,r,t)$, which is the market equilibrium price for user $i$ to receive its food from restaurant $r$ within tier $t$.



==> tex/others.tex <==
\subsection{Combinatorial Multi-Armed Bandit Approach}

Our first case of consideration is without any assumption on the structure of the matrix $R$. In this case, our problem maps to the setting of combinatorial multi-armed bandits. We can consider each allocation pair $(u, i)$ to be an arm with expected reward $R_{ui}$. In total, there are $N M$ arms and at each iteration we select of a subset of arms (a super arm in the context of CMAB). We are constrained to select a subset from $\mathcal{S} \in 2^{[NM]}$ where $\mathcal{S}$ corresponds to the allocations that comply with problem constraints. 

Let $r_R(X)$ denote the expected reward of an allocation $X$ when the reward matrix is given by $R$. Then, 
\begin{equation}
    r_R(X) = \sum_{u = 1}^{N} \sum_{i = 1}^{M} R_{ui} x_{ui}
\end{equation}

Then this reward structure satisfies the following properties:

\begin{enumerate}
    \item Monotonicity: If $R_{ui} \leq R_{ui}'$ for all $u \in [N], i \in [M]$, then we have $r_R(X) \leq r_{R'}(X)$
    \item Bounded smoothness: If $\max_{(u,i) \in [N]\times [M]} |R_{ui} - R_{ui}'| \leq \Lambda$, then we have $|r_R(X) - r_{R'}(X)| \leq N \Lambda$.
\end{enumerate}

\subsection{Low-Rank Multi-Armed Bandit \& Interactive Collaborative Filtering Approach}

Using the latent factor model (Hofmann and Puzicha 1999), the reward is assumed to be given by a product of user and item feature vectors $p_u$ and $q_i$:
\begin{equation}
    r_{ui} = p_u^\textrm{T}q_i + \eta
\end{equation}
where $\eta$ is a zero-mean Gaussian observation noise with variance $\sigma^2$.

\subsubsection{Distribution of User and Item Feature Vectors}

We adopt the PMF model (Salakhutdinov  and Mnih 2008) to build the distributions for the user and the item feature vectors, which are then used the generate the reward values. We define the prior distributions of the user and item feature vectors as Gaussian with variance $\sigma_p^2$
and $\sigma_q^2$:
\begin{align}
    p(p_u | \sigma_p^2) &= \mathcal{N}(p_u | 0, \sigma_p^2 I)\\
    p(q_i | \sigma_q^2) &= \mathcal{N}(q_i | 0, \sigma_q^2 I)
\end{align}

Then, the conditional distribution of the reward $r_{ui}$ given the user and item feature vectors follow a Gaussian distribution:
\begin{equation}
    p(r_{ui} | p_u, q_i, \sigma^2) =  \mathcal{N}(p_u^\textrm{T} q_i | 0, \sigma^2)
\end{equation}

By obtaining a set of noisy rating observations $\{u(k), i(k), r_{u(k) i(k)}\}_{k = 1}^{K}$, we can obtain the posterior distributions for the user and item feature vectors. Here, we first focus on the conditional distribution user feature vectors, given the current item feature vectors:
\begin{align}
    p(P | R, Q, \sigma^2, \sigma_p^2, \sigma_q^2) &= p(P | R, Q, \sigma^2, \sigma_p^2)\\
    &\propto p(R | P, Q, \sigma^2) \cdot p(P | \sigma_p^2)
\end{align}

